Zeroth-order non-convex learning via hierarchical dual averaging

We propose a hierarchical version of dual averaging for zeroth-order online non-convex optimization - i.e., learning processes where, at each stage, the optimizer is facing an unknown non-convex loss function and only receives the incurred loss as feedback. The proposed class of policies relies on the construction of an online model that aggregates loss information as it arrives, and it consists of two principal components: (a) a regularizer adapted to the Fisher information metric (as opposed to the metric norm of the ambient space); and (b) a principled exploration of the problem's state space based on an adapted hierarchical schedule. This construction enables sharper control of the model's bias and variance, and allows us to derive tight bounds for both the learner's static and dynamic regret - i.e., the regret incurred against the best dynamic policy in hindsight over the horizon of play.

==> App-Erratum.tex <==
%----------------------------------------------------------------------
%%% APP: ERRATUM
%----------------------------------------------------------------------
% !TEX root = ./Main.tex


When uploading the supplement, we noticed and corrected the following copy-editing typos in the body of our paper:
\begin{itemize}
\item
\textbf{Lines 272\textendash274, right:}
$\simple$ should read $\ppoint$

\item
\textbf{Line 323, left:}
There was an overload of $\simple$ in \eqref{eq:Fench-bound}, one of the $\simple$'s should read $\ppoint$.
The corrected equation is as follows:
\begin{equation*}
\fench(\base,\dpoint+\dvec)
	= \fench(\base,\dpoint)
		+ \braket{\dvec}{\ppoint - \base}
		+ \fench(\ppoint,\dpoint+\dvec)
	\leq \fench(\base,\dpoint)
		+ \braket{\dvec}{\ppoint - \base}
		+ \frac{1}{2\hstr} \norm{\dvec}_{\ppoint,\ast}^{2}
\end{equation*}

\item
\textbf{Line 299, right:}
There was a typo in the summation indices, the two sums should read $\sum_{\run\in\runs}$, not $\sum_{\run=\start}^{\nRuns}$.

\item
\textbf{Line 305, right:}
The bound should read $\abs{\braket{\bias_{\run}}{\simple}} \leq \bbound_{\run}$ for $\simple\in\simples_{\cover}$.

\item
\textbf{Line 322, right:}
$\temp_{\nRuns}^{-1}$ should read $\temp_{\nRuns+1}^{-1}$.

\item
\textbf{Line 357, right:}
Missing factor of $2$, the correct expression is $\diam(\set) \leq 2\diam(\points) \nSets_{\run}^{-1/\vdim}$.
%\PM{Please check.}

\item
\textbf{Lines 404 \& 414, right:}
Missing ``+'', the correct expressions should read $\nRuns^{1-\nSetsExp / \vdim} + \nRuns^{2\pexp-2\mexp}\tvar$ and $\nRuns^{1-\nSetsExp / \vdim} + \nRuns^{2\pexp-\nSetsExp}\tvar$.

\item
\textbf{Line 418, right:}
Missing ``$/$'', the value for $\pexp$ should read $\pexp = (1 - \vexp)(\vdim +1)/(\vdim + 3)$.
\end{itemize}
All these typos have been corrected herein.

%\TR{mention the correction missing in \eqref{eq:HDA} here?}
%\PM{Undecided atm \textendash\ WDYT?}
%\TR{not sure.. at least it is mentioned in the appendix :)}
%\PM{What I'm worried about is a reviewer complaining that we are ``restarting'' the algo. We are making a big fuss in the intro that we are \emph{not} restarting the algo, and this is because of the correction that we introduce \textendash\ so I think we should explain this in detail at some point\dots}


%\TR{3 typos for theorem 2 which do not change the big O bounds whatsoever}
%\TR{the terms involving the $\phi$ in theorem 2 will be slightly different}
%\TR{the $C_\theta$ will be next to a $\sigma_T$}
%\TR{There might be a factor 2 missing on the sum for the approximation}
%\TR{stating a result using partly done computation and intuition = dangerous haha}

%\PM{Eek, a minor point, but I just realized the symbol $\nSplits_\run$ looks like a ``variance''\dots WDYT?}\TR{damnit there are not enough letters..}

%\TR{In proposition 1 and theorem 1, should we take $\simple \in \simples_\cover$? Same question for the definition of the bias in (19a) should this be for all $\simple \in \simples_\cover$ where $\cover$ is the underlying partition used by \eqref{eq:DAX}?}
%\PM{Fixed.}

==> App-Test.tex <==
%----------------------------------------------------------------------
%%% APP: TEST
%----------------------------------------------------------------------
% !TEX root = ./Main.tex


Trying to adapt the X-bandit approach to Exp3.

$\points$ is covered by infinite binary tree (each node has two children).
The tree is such that any finite cut (we remove all children of some nodes, such that the tree is still binary but with a finite number of leaves) covers $\points$.
There are no intersection between leaves.
We also assume that the volume covered by a leaf is half of the volume covered by its parent.
\AH{on Xbandits papers they have finer assumptions}

We write the proof that will apply for a constant step size $\step$ as well as for a decreasing step size $\step_\run$.

We need the reward function $u$ to be in $[0,1]$.

\paragraph{\textbf{Algorithm}}

\begin{itemize}
    \item Start with the tree $\mathcal{T}$ with $k_0>0$ leaves the score of each leaf is $S_{0,i}=0$ for $i \in [0, k_0]$
    \item for $\run = 1, \ldots $:
    \begin{enumerate}
        \item Calculate the sampling distribution on leaves for $\play \in [0,k_\run]$:
        \[P_{\run,\play} = \frac{exp(\step_\run S_{\run-1,\play})}{\sum_{\playalt=1}^{k_\run}exp(\step_\run S_{\run-1,\playalt})}\]
        \item sample a leaf $L_{\run}$ according to the distribution,
        \item sample an action $\state_\run$ in $L_{\run}$,
        \item update $S_{\run,\play} = S_{\run-1,\play} +1 - \frac{1 - \pay_{\run}(\state_\run)}{P_{\run,\play}} \one_{\play =L_{\run}} $ for $\play \in [0,k_\run]$
        \item $k_{\run + 1} = k_{\run}$
        \item if $\run$ satisfies a given criterion :
        \begin{itemize}
            \item split a given leaf $L'_{\run}$ in its children : $(L'_{\run}, k_\run +1) \leftarrow L'_{\run}$
            \item $S_{\run,L'_{\run}} = S_{\run,L'_{\run}} - log(2/\step_\run)$ and $S_{\run,k_\run +1} = S_{\run,L'_{\run}} - log(2/\step_\run)$
            \item $k_{\run+1} = k_{\run} +1$
        \end{itemize}
    \end{enumerate}
\end{itemize}
The choice of the criterion to increase the number of leaves as well as which leaf to split will be analyse later.

\begin{figure}[h!]
\centering
\includegraphics[width=.5\textwidth]{Figures/tree_drawing.jpg}
\caption{Example of a tree. In red is the id of the node (when it was a leaf), in blue its diameter. The number below a node is the step at which it was split into its children. }
\end{figure}

\paragraph{\textbf{Notation and small calculus}}

To follow the proof of Exp3 (Lattimore) we note:
\begin{itemize}
    \item $\pay_{\run,L} =\ex_{\state \in L}[\pay_{\run}(\state)] $;
    \item $\est{\pay_{\run,L}} =\ex_{\state \in L}[\est{\pay_{\run}}(\state)] $;
    \item $\est{\pay_{\run,\play}}(\state_\run) = 1 -  \frac{1 - \pay_{\run}(\state_\run)}{P_{\run,\play}} \one_{\play =L_{\run}}$;
    \item $W_\run (\step) = \sum_{\play = 0}^{k_{\run+1}} exp(\step S_{\run,\play})= \sum_{\play = 0}^{k_{\run}} exp(\step S_{\run - 1,\play}) exp(\step \est{\pay_{\run,\play}}) $;
    \item $h_\run(\play)$ is the height of the leaf $\play$ at time $\run$.
\end{itemize}
Note that if $\play$ is higher that $k_{\run}$ then it refers to its parent that was a leaf at time $\run$.

We will use this small calculation results:
\begin{itemize}
    \item $\pay_{\run,\play} =  \ex_{L_{\run}\sim P_\run,\state \in \play }[\est{\pay_{\run,\play}} ] = \mathbb{E}_{\state \in \play}[\pay_{\run}(\state)] = \mathbb{E}_{L_{\run}\sim P_\run}[\est{\pay_{\run,L_{\run}}}]$
    \item $\pay_{\run,L_\run} =  \ex_{\play\sim P_\run,\state_{\run} \in L_\run }[\est{\pay_{\run,\play}} ]= \mathbb{E}_{\state \in  L_\run}[\pay_{\run}(\state)] = \mathbb{E}_{\play\sim P_\run}[\est{\pay_{\run,\play}}]$
    \item $\ex_{\play \sim P_\run}[\est{\pay}^2_{\run,\play}] = \frac{\pay^2_{\run,L_\run}}{P_{\run, L_\run}}$
    \item $\ex_{L_\run \sim P_\run}[\frac{1}{P_{\run, L_\run}}] = k_{\run}$
\end{itemize}
Here $\ex_{\play\sim P_\run}$ is purely computational as a shortcut of anything of type $\sum_{\play=0}^{k_\run} P_{\run,\play} Y(\play) = \ex_{\play\sim P_\run} Y(\play)$.

In the following we will often avoid to write the expectation on choosing an action among all the actions of a given leaf, it will be implicit, we will then use $\est{\pay_{\run,L}}$ instead of $\est{\pay_{\run}}(\state)$ (because we always end up taking the expectation).

\paragraph{\textbf{Preliminaries: Link between the regret of a leaf and the difference of scores}}

\begin{equation}
\begin{split}
    \exof{S_{\run,\play}} &=  \exof{S_{\run - 1 ,\play}} + \exof{\est{\pay_{\run,\play}} } - \frac{log(2)}{\step_\run} \one_{split, \play =L'_{\run}}\\
    & = \sum_{\runalt = 1}^{\run} \exof{\est{\pay_{\runalt,\play}} } - \frac{log(2)}{\step_\runalt} \one_{split(\runalt), \play =L'_{\runalt}}\\
    & = \sum_{\runalt = 1}^{\run} \pay_{\runalt,\play} - \sum_{\runalt = 1}^{\run}\frac{log(2)}{\step_\runalt} \one_{split(\runalt), \play =L'_{\runalt}}\\
    %& \geq \sum_{\runalt = 1}^{\run} \pay_{\runalt,\play} - h_\run(\play)\frac{log(2)}{\step_\run}
\end{split}
\end{equation}
Where $split(\runalt)$ means that there is a split at time $\runalt$ (it satisfies the criterion).

\begin{itemize}
    \item $S_\run = \sum_{\runalt = 1}^{\run} \exof{\est{\pay_{\runalt,L_\runalt}} } - \exof{\sum_{\runalt = 1}^{\run}\frac{log(2)}{\step_\runalt} \one_{split(\runalt), \play =L'_{\runalt}} } $
    \item $R_{\run, \play} = \sum_{\runalt = 1}^{\run} \exof{\est{\pay_{\runalt,\play}} } - \sum_{\runalt = 1}^{\run} \exof{\est{\pay_{\runalt,L_\runalt}} } \leq  \exof{S_{\run,\play}} - S_\run +\frac{log(2)}{\step_\run}  $ for all  $\play \in [0,k_\run]$ because the tree is such that two leaves have at most one difference of height and $(\step_\runalt)_\runalt$ is constant or decreasing.
\end{itemize}

The tricky part is to find an upper bound of $\exof{S_{\run,\play}} - S_\run$.

\paragraph{\textbf{Focus on bounding  $\exof{S_{\run,\play}} - S_\run$}}

Note that equation 11.11 still holds
\begin{equation}
    \frac{ W_{\runalt}}{W_{\runalt-1}}(\step_\runalt) = \sum_{\play = 0}^{k_{\runalt+1}} \frac{exp(\step_\runalt S_{\runalt,\play})}{W_{\runalt-1}(\step_\runalt)} = \sum_{\play = 0}^{k_{\runalt}} \frac{exp(\step_\runalt S_{\runalt-1,\play})exp(\step_\runalt \est{\pay_{\runalt,\play}})}{W_{\runalt-1}(\step_\runalt)} = \sum_{\play = 0}^{k_{\runalt}} P_{\runalt ,\play} exp(\step_\runalt \est{\pay_{\runalt,\play}})
\end{equation}
equation 11.12 still holds (we use $exp(x)\leq 1 + x + x^2/2$ and $x \leq exp (x-1)$ for $x\geq 0$) 

\begin{equation}
\begin{split}
    \frac{ W_{\runalt}}{W_{\runalt-1}}(\step_\runalt)&\leq 1 + \step_\runalt \sum_{\play = 0}^{k_{\runalt}} P_{\runalt ,\play}\est{\pay_{\runalt,\play}} + \step_\runalt^2 \sum_{\play = 0}^{k_{\runalt}} P_{\runalt ,\play}\est{\pay_{\runalt,\play}}^2 \\
    &\leq exp( \step_\runalt \sum_{\play = 0}^{k_{\runalt}} P_{\runalt ,\play}\est{\pay_{\runalt,\play}} + \step_\runalt^2 \sum_{\play = 0}^{k_{\runalt}} P_{\runalt ,\play}\est{\pay_{\runalt,\play}}^2)\\
    &\leq exp( \step_\runalt \ex_{\play\sim P_\runalt}[\est{\pay_{\runalt,\play}} ] + \step_\runalt^2 \ex_{\play \sim P_\runalt}[\est{\pay}^2_{\runalt,\play}])\\
    &\leq exp( \step_\runalt \ex_{\play\sim P_\runalt}[\est{\pay_{\runalt,\play}} ] + \step_\runalt^2 \frac{\pay^2_{\runalt,L_\runalt}}{P_{\runalt, L_\runalt}})\\
    \frac{1}{\step_\runalt} log(\frac{ W_{\runalt}}{W_{\runalt-1}}(\step_\runalt)) &\leq \ex_{\play\sim P_\runalt}[\est{\pay_{\runalt,\play}} ] + \step_\runalt \frac{\pay^2_{\runalt,L_\runalt}}{P_{\runalt, L_\runalt}} \leq \pay_{\runalt,L_\runalt} +  \frac{\step_\runalt}{P_{\runalt, L_\runalt}} \\
    - \pay_{\runalt,L_\runalt} &\leq - \frac{1}{\step_\runalt} log(\frac{ W_{\runalt}}{W_{\runalt-1}}(\step_\runalt)) +  \frac{\step_\runalt}{P_{\runalt, L_\runalt}}
\end{split}
\end{equation}

Now we will also follow the proof of Bubeck 2012 (http://sbubeck.com/SurveyBCB12.pdf) for EXP3 (theorem 3.1) to study the term $\frac{1}{\step_\runalt} log(\frac{ W_{\runalt}}{W_{\runalt-1}}(\step_\runalt))$.

Let $\Phi_\run(\step)= \frac{1}{\step}log\left(\frac{W_{\run}(\step)}{m_\run}\right)$ and $\Phi_0(\step)=0$, we will see that for the constant step size algorithm $m_\run=W_0= k_1$ such that $\Phi_0(\step)=0$. But for the decreasing step size algorithm we will need $m_\run = k_{\run +1}$, so far we will just assume that $m_\run$ is increasing.

\begin{equation}
\begin{split}
\frac{1}{\step_\runalt} log\left(\frac{ W_{\runalt}}{W_{\runalt-1}}(\step_\runalt)\right) &= \frac{1}{\step_\runalt} \left( log\left(\frac{W_{\runalt}(\step_\runalt)}{m_{\runalt}}\right) - log\left(\frac{W_{\runalt-1}(\step_\runalt)}{m_{\runalt-1}}\right) - log\left(\frac{m_{\runalt-1}}{m_{\runalt}}\right) \right) \\
&\geq  \Phi_\runalt(\step_\runalt) - \Phi_{\runalt-1}(\step_\runalt)
\end{split}
\end{equation}

Combining equations above we obtain 
\begin{equation}
    - \pay_{\runalt,L_\runalt} \leq  \Phi_{\runalt-1}(\step_\runalt) - \Phi_{\runalt}(\step_\runalt) +  \frac{\step_\runalt}{P_{\runalt, L_\runalt}}
\end{equation}

By summing we have:

\begin{equation}
\begin{split}
    - \sum_{\runalt=1} ^{\run} \pay_{\runalt,L_\runalt} &\leq \sum_{\runalt=1} ^{\run} \Phi_{\runalt-1}(\step_\runalt) - \Phi_{\runalt}(\step_\runalt) +  \frac{\step_\runalt}{P_{\runalt, L_\runalt}}\\
    &\leq \sum_{\runalt=1} ^{\run} \frac{\step_\runalt}{P_{\runalt, L_\runalt}} +  \sum_{\runalt=0} ^{\run-1}\Phi_{\runalt}(\step_{\runalt+1}) - \sum_{\runalt=1} ^{\run} \Phi_\runalt(\step_\runalt) \\
    &\leq \sum_{\runalt=1} ^{\run} \frac{\step_\runalt}{P_{\runalt, L_\runalt}} + \sum_{\runalt=1} ^{\run-1} \left( \Phi_\runalt(\step_{\runalt+1}) - \Phi_\runalt(\step_{\runalt})\right) - \Phi_\run(\step_\run)
\end{split}
\end{equation}

In the case of constant step size we have $\left( \Phi_\runalt(\step_{\runalt+1}) - \Phi_\runalt(\step_{\runalt})\right) =0$, in the case of decreasing step size, we show that $\Phi_\run(\step)$ is increasing.

\begin{equation}
\begin{split}
    \frac{d\Phi_\run(\step)}{d \step} &= \frac{- log\left(\frac{W_{\run}(\step)}{m_\run}\right)}{\step^2} + \frac{\sum_{\play = 0}^{k_{\run+1}}S_{\runalt,\play}exp(\step S_{\run,\play})}{\step \sum_{\play = 0}^{k_{\run+1}}exp(\step S_{\run,\play})}\\
    &= \frac{ \sum_{\playalt = 0}^{k_{\run+1}}exp(\step S_{\run,\playalt}) \left(  \step S_{\run,\playalt} -  log\left(\frac{\sum_{\play = 0}^{k_{\run+1}}exp(\step S_{\run,\play})}{m_\run}\right) \right)}{\step^2 \sum_{\play = 0}^{k_{\run+1}}exp(\step S_{\run,\play})}\\
    & = \frac{1}{\step^2} \sum_{\playalt = 0}^{k_{\run+1}} \frac{ exp(\step S_{\run,\playalt})}{\sum_{\play = 0}^{k_{\run+1}}exp(\step S_{\run,\play})} log\left( \frac{m_\run exp(\step S_{\run,\playalt})}{\sum_{\play = 0}^{k_{\run+1}}exp(\step S_{\run,\play})}  \right)
\end{split}
\end{equation}

When $m_\run=k_{\run+1}$ $\frac{1}{k_{\run+1}}$ is the uniform distribution over the $k_{\run+1}$ arms and $\frac{d\Phi_\run(\step)}{d \step}$ is the KL-divergence between the probability $\frac{ exp(\step S_{\run,\playalt})}{\sum_{\play = 0}^{k_{\run+1}}exp(\step S_{\run,\play})}$ and the uniform probability. 
The derivative is thus positive and the function is increasing.

Note that for $m_\run<k_{\run+1}$ the derivative is not always positive, for example if all $S_{\run,\playalt}$ are equal the derivative is negative.

Lets now rewrite the last term:

\begin{equation}
\begin{split}
    - \Phi_\run(\step_\run) &= -\frac{1}{\step_\run}log\left(\frac{W_{\run}(\step_\run)}{m_\run}\right) \\
    &= \frac{log(m_\run)}{\step_\run} - \frac{1}{\step_\run} log\left( \sum_{\play = 0}^{k_{\run+1}}exp(\step_\run S_{\run,\play}) \right) \\
    &\leq \frac{log(m_\run)}{\step_\run} - S_{\run,\play}
\end{split}
\end{equation}
And this is true for any $\play$ among the arms available at time $\run$.

Putting all together we have for all $\play$ :
\begin{equation}
   S_{\run,\play} - \sum_{\runalt=1} ^{\run} \pay_{\runalt,L_\runalt}\leq \sum_{\runalt=1} ^{\run} \frac{\step_\runalt}{P_{\runalt, L_\runalt}} + \frac{log(m_\run)}{\step_\run}
\end{equation}

Taking the expectation we obtain
\begin{equation}
    \exof{S_{\run,\play}} - S_\run \leq \sum_{\runalt=1} ^{\run} \step_\runalt k_\runalt + \frac{log(m_\run)}{\step_\run}
\end{equation}

Going back to the regret, we have:

\begin{equation}
    R_{\run, \play} \leq \frac{log(m_\run) + log(2)}{\step_\run} + \step_\run \sum_{\runalt=1}^{\run} (k_{\runalt}+ 1)
\end{equation}

%\paragraph{\textbf{Regret for continuous arm}}

%However we still don't have the regret for continuous arm:
%\begin{equation}
%    \begin{split}
%        R_\run &= max_{\state \in \points} \sum_{\runalt = 1}^{\run} u_{\runalt}(\state) - \sum_{\runalt = 1}^{\run} \exof{\est{\pay_{\runalt,L_\runalt}} } \\
%        &= max_{\state \in \points} \sum_{\runalt = 1}^{\run} u_{\runalt}(\state) - S_\run - log(2)\exof{h_\run(L_\run)})\\
%        &= max_{\state \in \points} \sum_{\runalt = 1}^{\run} u_{\runalt}(\state) - \exof{S_{\run,\play}} + \exof{S_{\run,\play}} - S_\run - log(2)\exof{h_\run(L_\run)})\\
%        &= max_{\state \in \points} \sum_{\runalt = 1}^{\run} u_{\runalt}(\state) - \sum_{\runalt = 1}^{\run} \pay_{\runalt,\play} + h_\run(\play)log(2)+\exof{S_{\run,\play}} - S_\run - log(2)\exof{h_\run(L_\run)})\\
%        R_\run &= max_{\state \in \points} \sum_{\runalt = 1}^{\run} u_{\runalt}(\state) - \sum_{\runalt = 1}^{\run} \pay_{\runalt,\play} + R_{\run, \play} \\
 %       R_\run &\leq max_{\state \in \points} \sum_{\runalt = 1}^{\run} u_{\runalt}(\state) - \sum_{\runalt = 1}^{\run} \pay_{\runalt,\play}+\frac{log(m_\run)}{\step_\run} + \step_\run \sum_{\runalt=1}^{\run} (k_{\runalt}+ 1) + log(2)
 %   \end{split}
%\end{equation}


\paragraph{\textbf{Difference between best reward and its leaf's reward expectation}}

Let $\state^*$ be the point of the maximum, let $L^*_\run$ be such that for all $\run$, $\state^*$ is in $L^*_\run $.

Let $D$ be the diameter of $\points$, the diameter of any leaf at height $h$ of the tree is $\frac{D}{2^{\left\lfloor h/d\right \rfloor}}
$.

Assume that functions $u$ are 1-Lipschitz, then we have.
\begin{equation}
    \begin{split}
        \sum_{\runalt = 1}^{\run} u_{\runalt}(\state^*) - \sum_{\runalt = 1}^{\run} u_{\runalt,L^*_\runalt} & \leq \sum_{\runalt = 1}^{\run} diam(L^*_\runalt) \\
        & = \sum_{\runalt = 1}^{\run} \frac{D}{2^{\left\lfloor h_{\runalt}(L^*_\runalt)/d \right \rfloor}}
    \end{split}
\end{equation}

Let assume that the tree is explored greedily independently of the rewards. We start with $k_0 = 0$ the root then we split the root. then we split each of its children. And so one so that the maximal and the minimal height are either equal or of the with a difference of one.

Let assume that we split a leaf if $\left\lfloor\run ^ {p}\right\rfloor = \left\lfloor(\run-1) ^ {p}\right\rfloor + 1$ with $p \in (0,1]$.

Therefore the tree is a complete binary tree of height $h$ for $\run = \left\lceil (2^{h}-1)^{1/p}\right\rceil$.

The minimal height of the tree is $h$ during $\left\lceil(2^{h+1}-1)^{1/p}\right\rceil - \left\lceil(2^{h}-1)^{1/p}\right\rceil \leq 1+(2^{h+1}-1)^{1/p} - (2^{h}-1)^{1/p}$ steps.

Let $h_\run$ be the minimal height of the tree at step $\run$, thus $(2^{h_\run}-1)\leq \run^p < (2^{h_\run+1}-1)$, and for $h_\run \geq 1$ we have $(2^{h_\run/p-1/p})\leq(2^{h_\run}-1)^{1/p}\leq \run$
Therefore, we have 
\begin{equation}
    \begin{split}
        \sum_{\runalt = 1}^{\run} u_{\runalt}(\state^*) - \sum_{\runalt = 1}^{\run} u_{\runalt,L^*_\runalt} &\leq \sum_{\runalt = 1}^{\run} \frac{D}{2^{\left\lfloor h_{\runalt}/d \right \rfloor}}\\
        & \leq \sum_{h = 0}^{h_{\run}} \frac{D}{2^{\left\lfloor h/d \right \rfloor}} (1+(2^{h+1}-1)^{1/p} - (2^{h}-1)^{1/p})\\
        & \leq \sum_{l = 0}^{\left\lfloor h_{\run}/d \right \rfloor +1} \frac{D}{2^l} (1+(2^{d(l+1)}-1)^{1/p} - (2^{dl}-1)^{1/p})\\
        & = \sum_{l = 0}^{\left\lfloor h_{\run}/d \right \rfloor +1} \frac{D}{2^l} + \sum_{l = 0}^{\left\lfloor h_{\run}/d \right \rfloor +1 } \frac{D}{2^l}(2^{d(l+1)}-1)^{1/p} - 1/2 \sum_{l = 0}^{\left\lfloor h_{\run}/d \right \rfloor} \frac{D}{2^{l}}(2^{d(l+1)}-1)^{1/p}\\
        &\leq 2D + \sum_{l = 0}^{\left\lfloor h_{\run}/d \right \rfloor} \frac{D}{2^{l+1}}(2^{d(l+1)}-1)^{1/p} + \frac{D}{2^{\left\lfloor h_{\run}/d \right \rfloor +1}}(2^{\left\lfloor h_{\run}/d \right \rfloor d+2d} - 1)^{1/p}\\
        &\leq2D + D\sum_{l = 0}^{\left\lfloor h_{\run}/d \right \rfloor} 2^{(l+1)(d/p-1)} + \frac{D}{2^{{\left\lfloor h_{\run}/d \right \rfloor}+1}}(2^{h_{\run}+2d}-1)^{1/p}\\
        &\leq 2D + D \int_{0}^{\left\lfloor h_{\run}/d \right \rfloor}exp(log(2)(l+1)(d/p-1))dl + \frac{D}{2^{{\left\lfloor h_{\run}/d \right \rfloor}+1}}(2^{h_{\run}+2d}-1)^{1/p}\\
        &\leq 2D + \frac{D}{log(2)(d/p-1)}2^{({\left\lfloor h_{\run}/d \right \rfloor}+1)(d/p-1)}+ \frac{D}{2^{{\left\lfloor h_{\run}/d \right \rfloor}+1}}(2^{h_{\run}+2d}-1)^{1/p}\\
        &\leq 2D + \frac{D}{2^{{\left\lfloor h_{\run}/d \right \rfloor}+1}}\left( \frac{2^{d/p}}{log(2)(d/p-1)} 2^{h_{\run}/p} +2^{h_{\run}/p +2d/p} \right)\\
        &\leq 2D + \frac{2D 2^{(2d+1)/p}}{t^{p/d}} t\\
        &\approx O(t^{(1-p/d)})
    \end{split}
\end{equation}

\paragraph{\textbf{Conclusion}}

Recall that $k_{\runalt}+ 1$ is the number of leaves at steps $\runalt$, therefore $\sum_{\runalt=1}^{\run} k_{\runalt}+ 1 \leq \sum_{\runalt=1}^{\run} \runalt^{p}= O(\run^{p+1}) $

All together we have

$R_\run = O(\run^{(1-p/d)}) + \frac{log(m_\run)+ log(2)}{\step_\run} + \step_\run O(\run^{p+1})$

If the step size is constant, we take $m_\run=W_0$ and the best parameters are $ p = \frac{d}{d+2}$ and $\step = T^{-\frac{p+1}{2}}= T^{-\frac{d+1}{d+2}}$ leading totane 
$R_T =O(T^{\frac{d+1}{d+2}})$

If the step size is decreasing, we take $m_\run=k_{\run+1}$ and the same best parameters, $\step_\run = \run^{-\frac{d+1}{d+2}}$ and $ p = \frac{d}{d+2}$, are optimal leading to
$R_T =O(log(T)T^{\frac{d+1}{d+2}})$

==> DualAvg-old.tex <==
%----------------------------------------------------------------------
%%% DUAL AVERAGING
%----------------------------------------------------------------------
% !TEX root = ./Main.tex


%The plan (under construction):
%\begin{enumerate}
%\item
%Finite case:
%	important for intuition / motivation,
%	playground for simple strategies (arm $\iff$ supporting set)
%\item
%Present dual averaging:
%	general mirror,
%	general models.
%Say that we detail everything below.
%
%\item
%The model:
%	to facilitate comparison of results, use \cite{HMMR20}),
%	present details
%
%\item
%The regularizer:
%	analysis of bandits with global norm can be too coarse,
%	need something more adapted when comparing distances between probability distributions
%	$\implies$ Fisher information metric
%
%\item
%Introduce assumptions for regularizer:
%	strong convexity relative to Fisher metric,
%	examples (Burg entropy, standard entropy),
%	discuss equivalence with strong smoothness of the conjugate,
%	relax assumption to hold over the range of the estimator.
%\end{enumerate}

To build some intuition for the analysis to come, we begin by adapting the classical \acdef{DA} algorithm to the space of simple strategies with an explicit cover.
This will allow us to introduce the relevant notions that we will need in the sequel, namely the \emph{range} of an estimator and the \emph{Fisher information metric}.


%----------------------------------------------------------------------
%%% DualAvg
%----------------------------------------------------------------------
\subsection{Basic setup}


When choosing actions from a finite set $\pures = \{1,\dotsc,\nPures\}$, our learning framework is modified as follows:
\begin{enumerate*}
[(\itshape i\hspace*{1pt}\upshape)]
\item
at each stage $\run=\running$, the adversary chooses (but does not reveal) a reward vector $\payv_{\run} \in \R^{\pures}$;
\item
the learner selects an action $\choice_{\run} \in \pures$;
and
\item
the corresponding reward $\est\pay_{\run} = \payv_{\choice_{\run},\run}$ is awarded to the learner and the process repeats.
\end{enumerate*}
Thus, in terms of our basic model, the payoff function encountered at stage $\run$ is $\pay_{\run}(\pure) = \payv_{\pure,\run}$, and we will assume that $\payv_{\pure,\run} \in [0,\rbound]$ for all $\run=\running$, and all $\pure\in\pures$.

In this setting, the \acdef{DA} algorithm amounts to the recursive action selection rule
\begin{equation}
\label{eq:DA}
\tag{DA}
\begin{aligned}
\score_{\run+1}
	&= \score_{\run} + \model_{\run}
	\\
\choice_{\run+1}
	\sim \state_{\run+1}
	&= \mirror(\learn_{\run+1} \score_{\run+1})
\end{aligned}
\end{equation}
where

\begin{enumerate}
[itemsep=0pt]

\item
$\model_{\run}$ is an \emph{estimate} \textendash\ or \emph{model} \textendash\ of the otherwise unobserved reward vector $\payv_{\run} \in \R^{\nPures}$ of stage $\run$.

\item
$\score_{\run}$ is an auxiliary \emph{score} variable that aggregates previous payoff estimates \textendash\ so $\score_{\pure,\run}$ corresponds to the learner's propensity of choosing $\pure\in\pures$ at stage $\run$. 

\item
$\mirror\from\R^{\pures} \to \strats$ is a \emph{choice map} that transforms scores into actual mixed strategies $\state_{\run} \in \strats$.

\item
$\learn_{\run} > 0$ is a ``learning rate'' parameter that adjusts the sharpness of the learning process.
\end{enumerate}

Each component of the method is discussed in detail below.
We also note that, in the online learning literature, this method is often referred to as \acdef{FTRL}, and it is closely related to \acl{OMD}, \cf \citet{SS11,SSS06}.
Our choice of terminology follows \citet{Nes09} and \citet{Xia10}.


%----------------------------------------------------------------------
%%% EXP3 base
%----------------------------------------------------------------------
\subsection{Estimators}

We begin by detailing the estimate $\model_{\run}$ of the learner's reward vector $\payv_{\run}$ at time $\run$.
For generality, we will assume that this estimate is of the general form
\begin{equation}
\label{eq:model}
\model_{\run}
	= \payv_{\run}
		+ \error_{\run},
\end{equation}
where $\error_{\run} \in \R^{\pures}$ is a generic ``observation error'' that captures all sources of uncertainty in the learner's estimation process.
To differentiate between random (zero-mean) and systematic (nonzero-mean) errors, we will further decompose $\error_{\run}$ as
\begin{equation}
\label{eq:error}
\error_{\run}
	= \noise_{\run}
		+ \bias_{\run},
\end{equation}
where
\begin{equation}
\label{eq:bias-noise}
\bias_{\run}
	= \exof{\error_{\run} \given \filter_{\run}}
	\quad
	\text{and}
	\quad
\exof{\noise_{\run} \given \filter_{\run}}
	= 0,
\end{equation}
with $\filter_{\run} \defeq \filter(\pure_{1},\dotsc,\choice_{\run})$ denoting the history of the learner's actions up to \textendash\ and including \textendash\ stage $\run$.%
\footnote{In terms of the sequence of events described earlier, this means that $\choice_{\run}$ is $\filter_{\run}$-measurable, but $\error_{\run}$, $\noise_{\run}$ and $\bias_{\run}$ are not.}
For concreteness, we provide some examples below:

%We may then characterize the error in the estimator $\model_{\run}$ by means of the following statistics:
%\begin{subequations}
%\label{eq:sigbounds}
%\begin{alignat}{3}
%\label{eq:bbound}
%a)
%	\quad
%	&\textit{Bias:}
%	&\hspace{1em}
%	\bbound_{\run}
%		&= \exof{\dnorm{\bias_{\run}} \given \filter_{\run}}
%	\\
%\label{eq:variance}
%b)
%	\quad
%	&\textit{Variance:}
%	&\hspace{1em}
%	\sdev_{\run}^{2}
%		&= \exof{\dnorm{\noise_{\run}}^{2} \given \filter_{\run}}
%	\\
%\label{eq:mbound}
%c)
%	\quad
%	&\textit{Mean square:}
%	&\hspace{1em}
%	\mbound_{\run}^{2}
%		&= \exof{\dnorm{\model_{\run}}^{2} \given \filter_{\run}}
%	\hspace{4em}
%\end{alignat}
%\end{subequations}
%where $\norm{\cdot}$ is an arbitrary norm on $\R^{\pures}$ and $\dnorm{\cdot}$ is its dual.

%----------------------------------------------------------------------
\begin{example}
[Parametric estimation]
Suppose that the reward vector encountered at stage $\run$ is of the form $\payv_{\run} = \payv(\seed_{\run})$ for some
%parametric model $\payv\from\R^{\nCoords}\to[-\lbound,\lbound]$ and a
vector of parameters $\seed_{\run} \in \R^{\nCoords}$, possibly chosen adversarially at each stage.
In many cases of interest (\eg in online path planning, \cf \citealp{CBL12}), the learner observes an estimate $\est\seed_{\run}$ of $\seed_{\run}$, leading to the estimator $\model_{\run} = \payv(\est\seed_{\run})$.
The bias, variance and mean square of $\payv_{\run}$ are then determined by the regularity of the parametric model $\payv(\seed)$ and the corresponding statistics of the observed estimate $\est\seed_{\run}$.
\end{example}
%----------------------------------------------------------------------


%----------------------------------------------------------------------
\begin{example}
[\Acl{IWE}]
In the worst-case scenario where only the learner's reward $\est\pay_{\run} = \payv_{\choice_{\run},\run}$ is observed, a popular way to reconstruct $\payv_{\run}$ is via the \acli{IWE}
\begin{equation}
\label{eq:IWE}
\tag{\acs{IWE}}
\model_{\pure,\run}
	= \rbound
		- \oneof{\pure = \choice_{\run}} \frac{\rbound - \est\pay_{\run}}{\state_{\pure,\run}},
\end{equation}
which has been normalized here to take values in the region $\region = (-\infty,\rbound] \times \dotsm \times (-\infty,\rbound] \subseteq \R^{\pures}$.
A straightforward calculation shows that \eqref{eq:IWE} is \emph{unbiased} ($\exof{\model_{\run}} = \payv_{\run}$) and its variance is bounded as $\exof{(\model_{\pure,\run} - \payv_{\pure,\run})^{2}} = \bigoh(1/\state_{\pure,\run})$.
\PM{Can someone check me?}
This estimator plays a central role in bandit theory \citep{BCB12,Sli19,LS20}, and we will revisit it several times below.
\end{example}
%----------------------------------------------------------------------


%----------------------------------------------------------------------
\begin{example}
[\Acl{IWE3}]
One shortfall of \eqref{eq:IWE} is that it requires knowledge of the upper bound $\rbound$ for the learner's rewards.
This can be overcome by introducing an \emph{explicit exploration} parameter $\mix_{\run} > 0$ in the learner's sampling strategy and choose an action $\choice_{\run}\in\pures$ according to the perturbed strategy
\begin{equation}
\label{eq:explicit}
\est\state_{\run}
	= (1-\mix_{\run}) \state_{\run} + \mix_{\run} \unif_{\pures}.
\end{equation}
%where $\unif_{\pures}$ denotes the uniform distribution on $\pures$.
The \acli{IWE3} is then defined as
\begin{equation}
\label{eq:IWE3}
\tag{\acs{IWE3}}
\model_{\pure,\run}
	= \oneof{\pure = \choice_{\run}} \frac{\est\pay_{\run}}{\state_{\pure,\run}}.
\end{equation}
By construction, this estimator takes values in the region $\region = [0,\infty) \times [0,\infty)$;
in contrast to \eqref{eq:IWE}, the estimator \eqref{eq:IWE3} has bias $\exof{\model_{\pure,\run} - \payv_{\pure,\run}} = \bigoh(\mix_{\run})$ and variance bounded as $\exof{(\model_{\pure,\run} - \payv_{\pure,\run})^{2}} = \bigoh(1/\mix_{\run})$.
This estimator has reduced variance relative to \eqref{eq:IWE}, but the introduction of the explicit exploration parameter $\mix_{\run}$ introduces a further term in the regret (which is an important disadvantage).
\end{example}
%----------------------------------------------------------------------

Other possibilities also exist, such as \emph{implicit} exploration \needref, each with its own advantages and disadvantages;
\PM{Need to cite stuff here.}
for a detailed discussion, see \citet{Sli19}.



%----------------------------------------------------------------------
%%% Choice map
%----------------------------------------------------------------------
\subsection{The choice map}

The second component of \eqref{eq:DA} is the method's ``choice map'' $\mirror\from\R^{\pures} \to \strats$ which assigns probability to a given action $\pure\in\pures$ based on its score.
Specifically, the method outputs at each stage a mixed strategy $\state_{\run}\in\strats$ that maximizes the learner's expected propensity score minus a regularization penalty.

Specifically, we will consider choice maps of the form
\begin{equation}
\label{eq:choice}
\mirror(\dpoint)
	= \argmax_{\strat\in\strats} \braces{ \braket{\dpoint}{\strat} - \hreg(\strat) }
	\quad
	\text{for all $\dpoint\in\R^{\pures}$},
\end{equation}
where the \emph{regularizer} $\hreg\from\strats\to\R$ is assumed to be continuous and strongly convex on $\strats$, \ie for all $\strat,\stratalt\in\strats$, we have
\begin{equation}
\label{eq:strong}
\hreg(\coef\strat + (1-\coef)\stratalt)
	\leq \coef \hreg(\strat)
		+ (1-\coef) \hreg(\stratalt)
		- \tfrac{\hstr}{2} \coef(1-\coef) \norm{\stratalt - \strat}^{2},
\end{equation}
for some reference norm $\norm{\cdot}$ on $\R^{\pures}$ and some positive constant $\hstr>0$.

Two popular choices for $\mirror$ are the logit map
\begin{equation}
\label{eq:logit}
\logit(\dpoint)
	= \frac{(\exp(\dpoint_{1}),\dotsc,\exp(\dpoint_{\nPures}))}{\sum_{\pure=1}^{\nPures} \exp(\dpoint_{\pure})}
\end{equation}
and the Euclidean projector $\Eucl(\dpoint) = \argmin_{\strat\in\strats} \twonorm{\dpoint - \strat}$.
These choice maps are generated respectively by
the (negative) Snannon entropy $\hreg(\strat) = \sum_{\pure\in\pures} \strat_{\pure} \log\strat_{\pure}$ on $\strats$ (which is $1$-strongly convex relative to $\onenorm{\cdot}$),
and
the Euclidean regularizer $\hreg(\strat) = \twonorm{\strat}^{2}/2$ (which is $1$-strongly convex relative to $\twonorm{\cdot}$).
For a detailed discussion and a range of relevant examples, see \citet{Nes09}.


%----------------------------------------------------------------------
%%% Choice map
%----------------------------------------------------------------------
\subsection{Regret guarantees}

As we show below, the reference norm $\norm{\cdot}$ and the strong convexity modulus of $\hreg$ play a major role in the analysis of \eqref{eq:DA}.
This is because of the following ``template bound'' that can be derived for \eqref{eq:DA}

\PM{To be filled in with some template bound.}





==> Fisher.tex <==
%----------------------------------------------------------------------
%%% FISHER
%----------------------------------------------------------------------
% !TEX root = ./Main.tex


Closer inspection of the 

==> Tables/Related.tex <==
%----------------------------------------------------------------------
%%% PARAMETERS
%----------------------------------------------------------------------
% !TEX root = ../Main.tex


\begin{tabular}{r||lr||lr}
	&\textbf{Convex losses}
	&
	&\textbf{Non-Convex losses}
	&
	\\
\textbf{Feedback}
	&Static regret
	&Dynamic regret
	&Static regret
	&Dynamic regret
	\\
\hline
Exact
	&$\bigoh\parens[\big]{\nRuns^{1/2}}$
	&$\bigoh\parens[\big]{\nRuns^{2/3}\tvar^{1/3}}$
	&$\bigoh\parens[\big]{\nRuns^{1/2}}$
	&$\boldsymbol{\bigoh\parens[\big]{\nRuns^{2/3}\tvar^{1/3}}}$
	\\
\hline
Unbiased
	&$\bigoh\parens[\big]{\nRuns^{1/2}}$
	&$\bigoh\parens[\big]{\nRuns^{2/3}\tvar^{1/3}}$
	&$\boldsymbol{\bigoh\parens[\big]{\nRuns^{1/2}}}$
	&$\boldsymbol{\bigoh\parens[\big]{\nRuns^{2/3}\tvar^{1/3}}}$
	\\
\hline
Bandit
	&$\bigoh\parens[\big]{\nRuns^{1/2}}$
	&$\bigoh\parens[\big]{\nRuns^{4/5}\tvar^{1/5}}$
	&$\boldsymbol{\bigoh\parens[\big]{\nRuns^{\frac{\vdim+2}{\vdim+3}}}}$
	&$\boldsymbol{\bigoh\parens[\big]{\nRuns^{\frac{\vdim+3}{\vdim+4}}\tvar^{\frac{1^{\vphantom{1}}}{\vdim+4}}}}$
	\\
\hline
\end{tabular}

==> Thanks.tex <==
%----------------------------------------------------------------------
%%% THANKS
%----------------------------------------------------------------------
% !TEX root = ./Main.tex
%
%
This research was partially supported by the COST Action CA16228 ``European Network for Game Theory'' (GAMENET).
P.~Mertikopoulos is also grateful for financial support by
the French National Research Agency (ANR) under grant no.~ANR\textendash 16\textendash CE33\textendash 0004\textendash 01 (ORACLESS),
and the framework of the ``Investissements d’avenir'' program (ANR-15-IDEX-02) and the LabEx PERSYVAL (ANR-11-LABX-0025-01.
Zhengyuan Zhou is grateful for the IBM Goldstine fellowship.
